A Mini-Block Fisher Method for Deep Neural Networks

Deep neural networks (DNNs) are currently predominantly trained using first-order methods. Some of these methods (e.g., Adam, AdaGrad, and RMSprop, and their variants) incorporate a small amount of curvature information by using a diagonal matrix to precondition the stochastic gradient. Recently, effective second-order methods, such as KFAC, K-BFGS, Shampoo, and TNT, have been developed for training DNNs, by preconditioning the stochastic gradient by layer-wise block-diagonal matrices. Here we propose a "mini-block Fisher (MBF)" preconditioned gradient method, that lies in between these two classes of methods. Specifically, our method uses a block-diagonal approximation to the empirical Fisher matrix, where for each layer in the DNN, whether it is convolutional or feed-forward and fully connected, the associated diagonal block is itself block-diagonal and is composed of a large number of mini-blocks of modest size. Our novel approach utilizes the parallelism of GPUs to efficiently perform computations on the large number of matrices in each layer. Consequently, MBF's per-iteration computational cost is only slightly higher than it is for first-order methods. The performance of our proposed method is compared to that of several baseline methods, on both autoencoder and CNN problems, to validate its effectiveness both in terms of time efficiency and generalization power. Finally, it is proved that an idealized version of MBF converges linearly.

==> Neurips/sections/not.tex <==

\section{Notation and Definitions}

 Consider a deep neural network that transforms its input $x$ to an output $f(\bm{W};\bm{x})$ through a series of $L$ layers where $\bm{W}$ is the vector of network parameters. During the forward pass,  layer $l$ performs a linear transformation on its input of $m$ samples, i.e.  $\mathcal{I}_{l} \in \mathbb{R}^{d_i^l \times m}$,  parameterized with $\bm{W}_{l} \in \mathbb{R}^{d_i^l \times d_o^l}$,  and computes its outputs or \textit{pre-activations}, $\mathcal{O}_{l} = \bm{W}_{l}^\top \mathcal{I}_{l}$, followed by a nonlinear activation function such as ReLU.  The optimal parameters are obtained by minimizing the average loss $\Lb$ over the training set during the backward pass:
\begin{equation}
{\small
    \Lb(\bm{W}) = \frac{1}{n}\sum_{i=1}^n \ell (f(\bm{W};\textbf{x}_i), \textbf{y}_i)
    \label{eq:loss_equation}
    }
\end{equation}
where $\bm{W} \in \mathbb{R}^p$ is the vector containing all of the network’s parameters concatenated together, i.e. $[\text{vec}(\bm{W}_{1})^\top \text{vec}(\bm{W}_{2})^\top ... \text{vec}(\bm{W}_{L})^\top]^\top$, $\text{vec}(M)$ is the operator which vectorizes matrix $M$ by stacking columns together, and  $\ell$ measures the accuracy of the prediction (e.g. cross entropy loss).


\textbf{Gradient in DNN}:
 The average gradient over mini-batch $m$ is defined as $\bm{g} = \frac{1}{m}\sum_{i=1}^{m}\nabla_{\bm{W}}\ell (f(\bm{W};\textbf{x}_i), \textbf{y}_i)$ which is  obtained using standard backpropagation. In the backpropagation, each layer $l$ receives the gradient w.r.t its output, i.e. the \textit{pre-activation derivatives} $\mathcal{G}_l\in \mathbb{R}^{d_o^l \times m}$, and computes the gradient w.r.t its parameters, i.e. $\bm{g}_l = \frac{1}{m} \mathcal{I}_l \mathcal{G}_l^\top$. 


\textbf{Jacobian in DNN}:
The Jacobian of loss w.r.t the parameters for a single output network is defined as $\bm{J} = [\bm{J}_1^{\top}, ..., \bm{J}_n^{\top}]^\top \in \mathbb{R}^{n \times p}$ where $\bm{J}_i$ is the gradient of loss w.r.t the parameters. In the stochastic setting, for a layer $l$ the Jacobian of loss w.r.t  the layer parameters is approximated via $\bm{J}_l = (\mathcal{I}_l \ast \mathcal{G}_l)^\top \in \mathbb{R}^{m \times d_i^l d_o^l}$. 


\textit{ \textbf{NGD update rule}}. Natural gradient descent scales the gradient with the inverse of FIM as follows:
\begin{equation}
{\small
    \bm{W}(k+1) = \bm{W}(k) - \eta \left(\bm{F}(\bm{W}(k))  + \alpha \bm{I}\right)^{-1} \bm{g}(k)
    \label{eq:update_rule_fisher}
    }
\end{equation} 
 where $\eta$ is the learning rate, $\alpha$ is the damping parameter, $\bm{{F}}$ is the FIM of the model's conditional distribution $P_{\textbf{y}|\textbf{x}}$ and is defined as $\bm{{F}} = \mathbb{E}_{ P_{(\textbf{x},\textbf{y})}}[\nabla_{\bm{W}} \log p_{\bm{W}} (\textbf{y}|\textbf{x}) \nabla_{\bm{W}} \log p_{\bm{W}} (\textbf{y}|\textbf{x})^\top]$  where $p_{\bm{W}}$ is the model's density function. As shown in \cite{martens2020new}, the FIM coincides with Gauss-Newton matrix if the conditional distribution is in the exponential family which implies:
\begin{equation}
{\small 
    \bm{{F}} (\bm{W}(k)) = {\frac{1}{m}\sum_{i=1}^n \nabla_{\bm{W}} \ell_i {\nabla_{\bm{W}} \ell_i}^\top \big|_{
    \bm{W} = \bm{W}(k)}} = \frac{1}{n} \bm{J}(k)^\top \bm{J}(k) 
}
    \label{eq:fisher_matrix}
\end{equation}
where $\ell_i = \ell(f(\bm{W};\textbf{x}_i),\textbf{y}_i)$, $\bm{J}^{\bm{W}}(k)=[\bm{J}^{\bm{W}}_1(k)^\top,...,\bm{J}^{\bm{W}}_n(k)^\top]^\top$ and $\bm{J}^{\bm{W}}_i(k) = \nabla_{\bm{W}} \ell_i \big|_{
    \bm{W} = \bm{W}(k)}$. Hereafter, we use  $  \bm{{F}} (k) = \bm{{F}} (\bm{W}(k))$ to simplify the notations.

\textit{\textbf{Notations}}. Following notations are used in the paper:  $[L]:=\{1,...,L\}$, $\text{Diag}_{i=[L]}(A_i)$ is the block diagonal matrix with matrices $\{A_1,...,A_L\}$ on its diagonal; $\bm{X}\in\mathbb{R}^{n\times d}$ is the input data, i.e. $\bm{X}=[x_1,...,x_n]^\top$.  $\lambda_{\min}(M)$ is the smallest eigenvalue of  matrix $M$; Hadamard product between two matrices is  $\odot$;  the  Kronecker product is $\otimes$;  $\Vert.\Vert_2$ for the Euclidean norm of vectors/matrices; and $\ast$ is for the column-wise Khatri-Rao product; $A_{:i}$ is used to denote the $i$-th columns of matrix $A$.


